PREME: Preference-based Meeting Exploration through an Interactive Questionnaire

The recent increase in the volume of online meetings necessitates automated tools for managing and organizing the material, especially when an attendee has missed the discussion and needs assistance in quickly exploring it. In this work, we propose a novel end-to-end framework for generating interactive questionnaires for preference-based meeting exploration. As a result, users are supplied with a list of suggested questions reflecting their preferences. Since the task is new, we introduce an automatic evaluation strategy. Namely, it measures how much the generated questions via questionnaire are answerable to ensure factual correctness and covers the source meeting for the depth of possible exploration.

==> 06-limitations.tex <==
\section{Limitations}
\label{sec:limit}
Our work has the following limitations:
\begin{itemize}
    \item the use of GPT-3 can be potentially generate unrealistic questions, but we have accounted for that by introducing the metric for finding an answer;
    \item for human evaluation we hire two judges for evaluation;
\end{itemize}
